Geometric studies of the interplay between spin and gravity

This PhD thesis is the conclusion of some of my works carried out at the Centre de Physique Th\'eorique, under the supervision of Serge Lazzarini. Two subjects are presented in the manuscript, both aiming at studying the effect of the spin of elementary particles on otherwise known theories. First is a study of the L\'evy-Leblond-Newton (LLN) equation, which is used to describe the evolution of a quantum system with spin 1/2 that is coupled to its own gravitational potential. After reviewing some symmetries of non relativistic Quantum Mechanics, and how to geometrize them with the help of Bargmann structures, we recall what is the L\'evy-Leblond equation. In this chapter, the LLN equation is described in a fully covariant way on Bargmann structures. This covariant formulation then helps to derive the dynamical symmetries of the equation, and conserved quantities. The symmetry group of this equation turns out to be the already known Schr\"odinger-Newton group. The second part deals with the trajectory of particles with spin in General Relativity. We first highlight Souriau's geometric method to derive the Mathisson-Papapetrou-Dixon (MPD) equations, and then discuss the different possible Spin Supplementary Conditions (SSC) that exist to close the system of MPD equations. In this chapter, we assume the Tulczyjew SSC to describe the trajectory of photons, leading to the Souriau-Saturnini equations. We then present some works where we have applied these equations, in a Schwarzschild spacetime, and in a spacetime deformed by a gravitational wave. In the first work, we found gravitational birefringence: the trajectory deviates from the geodesic plane, depending on the helicity of the photon and its wavelength. The second work presented also found birefringence in gravitational interferometry experiments, however the effect is many orders of magnitude lower than what we can detect.

==> tex/chap3.tex <==
\chaptertoc{}

\section{Modèles}

	%% tableau nécessitant des filets verticaux
	\begin{table}[h!tbp]
		\begin{center}
			\begin{tabular}{c|*{5}{c}}
			0\\
			$c_2$    & $a_{21}$\\
			$c_3$    & $a_{31}$ & $a_{32}$\\
			$\vdots$ & $\vdots$ &           & $\ddots$\\
			$c_s$    & $a_{s1}$ & $a_{s2}$  & $\cdots$ & $a_{s,s - 1}$\\
			\hline
			         & $b_1$    & $b_2$     & $\cdots$ & $b_{s-1}$     & $b_s$\\
			\end{tabular}
		\end{center}
		\caption{Tableau de Butcher}
		\label{table:butcher}
	\end{table}

	%% tableau avec booktabs (sans filets verticaux)
	\begin{table}[h!tbp]
		\begin{center}
			\begin{tabular}{@{}lcc@{}} \toprule
			$\lambda$ (nm) & $(\alpha_{\lambda}/\alpha_{426,7})_{moy}$ & écart type \\ \midrule
			391,9 \& 392,1 & 0,12 & 0,01 \\
			588,9 \& 589,2 & 0,45 & 0,07 \\
			657,8 \& 658,3 & 6,70 & 0,06 \\
			711,3 & 0,16 & 0,01 \\
			711,6 & 0,15 & 0,01 \\
			712 & 0,31 & 0,02 \\ \bottomrule
			\end{tabular}
		\end{center}
		\caption[Valeur moyenne et écart type des rapports $\alpha_{\lambda}/\alpha_{426,7}$]{Valeur moyenne et écart type des rapports $\alpha_{\lambda}/\alpha_{426,7}$ mesurés pour les chocs plasma de la deuxième série.}
		\label{table:alpha}
	\end{table}

%\newpage

\section{Articles}

	\fullcite{mohamed_clinical_2014}
	% avant d'intégrer un article dans votre thèse, consulter http://www.sherpa.ac.uk/romeo/ si vous souhaitez diffuser sur internet
	\includepdfset{pagecommand=\thispagestyle{scrheadings}} % ajoute la numérotation continue des pages aux fichiers pdf importés
	\includepdf[scale=0.9,pages=-]{BMC-1471-2334-14-S2-O1.pdf} % 'scale' ajuste la taille du pdf, vous pouvez affiner en fonction des marges


==> tex/gloss.tex <==
%%% Acronymes

\newacronym{bc}{BC}{band contrast}

\newacronym{asb}{ASB}{bande de cisaillement adiabatique --ou \emph{Adiabatic Shear Band}--}


%%% Définitions (glossaire standard)

\newglossaryentry{rutile}{
	name={rutile},
	description={Espèce minérale composée de dioxyde de titane (\ce{TiO2}) et de traces de fer},
	}
	

%%% Nomenclature	

\newglossaryentry{+a}{
  type=notation,
  name={$+a$},
  description={Opérateur},
  sort={aaa}
}

\newglossaryentry{2a}{
  type=notation,
  name={$2a$},
  description={Nombre},
  sort={aab}
}

\newglossaryentry{ca}{
  type=notation,
  name={$:a$},
  description={Symbole de ponctuation},
  sort={aac}
}

\newglossaryentry{Aa}{
  type=notation,
  name={$Aa$},
  description={Lettre majuscule},
  sort={aad}
}

\newglossaryentry{aa}{
  type=notation,
  name={$aa$},
  description={Lettre minuscule},
  sort={aae}
}

\newglossaryentry{alpha}{
  type=notation,
  name={$\alpha$},
  description={Lettre grecque},
  sort={aaf}
}

